OMPar: Automatic Parallelization with AI-Driven Source-to-Source Compilation

Manual parallelization of code remains a significant challenge due to the complexities of modern software systems and the widespread adoption of multi-core architectures. This paper introduces OMPar, an AI-driven tool designed to automate the parallelization of C/C++ code using OpenMP pragmas. OMPar integrates Large Language Models (LLMs) through two key components: OMPify, which assesses loop parallelization potential, and MonoCoder-OMP, a new fine-tuned model which generates precise OpenMP pragmas. The evaluation of OMPar follows the same rigorous process applied to traditional tools like source-to-source AutoPar and ICPC compilers: (1) ensuring the generated code compiles and runs correctly in serial form, (2) assessing performance with the gradual addition of threads and corresponding physical cores, and (3) verifying and validating the correctness of the code's output. Benchmarks from HeCBench and ParEval are used to evaluate accuracy and performance. Experimental results demonstrate that OMPar significantly outperforms traditional methods, achieving higher accuracy in identifying parallelizable loops and generating efficient pragmas. Beyond accuracy, OMPar offers advantages such as the ability to work on partial or incomplete codebases and the capacity to continuously learn from new code patterns, enhancing its parallelization capabilities over time. These results underscore the potential of LLMs in revolutionizing automatic parallelization techniques, paving the way for more efficient and scalable parallel computing systems.

==> misc.tex <==
%The \tokom{} tokenization process involves generating an anonymized version of the original code by replacing variable names, numbers, and strings; parsing this anonymized code to create an Abstract Syntax Tree (AST); updating the AST to reflect anonymization changes and maintaining a change dictionary; converting the modified AST back into code while discarding extraneous details; splitting multi-part tokens like variable names for improved understanding; and attaching random numbers from a predefined range to recurring tokens to reduce reliance on specific replacements. This approach enhances a language model's comprehension of code structure and context, enabling better generalization and accurate code completions for high-performance computing, with the added benefit of being able to restore semantics using the change dictionary for user-friendly results.

% The Tokompiler tokenization process goes as follows:
% \begin{itemize}[wide, labelwidth=!, labelindent=0pt]

% \item \textit{Generate Replaced Code}: Create a version of the original code with anonymized variable names, numbers, and strings.
   
% \item \textit{AST Parsing}: Parse the anonymized code using tree-sitter or any suitable parser to generate an AST.

% \item \textit{Recreate AST Changes}: Update the AST to reflect the changes made during anonymization. Keep a dictionary of all changes done per file/function to facilitate restoring semantics back later.

% \item \textit{AST to Code-Tokenize}: Transform the updated AST back into code, eliminating any comments, new lines, and READMEs that may have been introduced during anonymization. This code-tokenized version will have a much smaller number of tokens.

% \item \textit{Token Splitting}: Split multi-part tokens (e.g., "var\_1" to ["var", "1"]) to ensure that the model comprehends variable names as a combination of type and a unique identifier.

% \item \textit{Random Number Attachment}: For recurring tokens (e.g., "var\_1" or "num\_2"), use statistics to attach random numbers from a predefined range (e.g., 1 to 1000) during each tokenization. The attached numbers are randomly chosen without any relation to the type or order of the replaced tokens or the file/function length.

% \end{itemize}

% By following this process, we can ensure that the model focuses on the code structure, context, and relevant semantics rather than learning specific local, unnecessary, or misleading semantics. Using random numbers and splitting tokens helps disentangle the importance of specific replacements from their roles as variables or arrays. This approach improves generalization and better code completions for high-performance code. Additionally, restoring semantics back to the user using the dictionary of changes at inference maintains the usability and interpretability of the model's results.


%Our work is also a first step towards improving the interpretability and explainability of code generated from LLMs, which are paramount for HPC practitioners to trust and validate the outcomes \cite{gottschlich2018three}.
%First, the enormous computational and memory requirements of LLMs pose a significant obstacle in their practical adoption for HPC languages and tasks \cite{xu2022systematic, li2023starcoder}. These models are often prohibitively large and demand substantial computational resources, making their deployment on standard HPC platforms challenging. Furthermore, adapting LLMs to specific HPC domains and ensuring their reliable generalization across diverse scientific and engineering applications demands further investigation \cite{yeticstiren2023evaluating, godoy2023evaluation, martinez2023code, guo2023longcoder, mukherjee2023stack}. Additionally, the interpretability and explainability of LLM-generated results are paramount for HPC practitioners to trust and validate the outcomes \cite{gottschlich2018three}.

%Ensuring reliable generalization of LLMs across diverse scientific and engineering HPC applications\footnote{Leveraging code LLMs for HPC tasks can speed up code development, generate optimized parallel implementations from high-level specifications, improve code readability and maintainability, facilitate cross-platform compatibility through code translation, optimize code for parallel execution and resource utilization, identify performance bottlenecks and parallelization issues, enable code search for existing optimized implementations, detect code duplication and bugs, suggest performance improvements, facilitate correct API usage, analyze code dependencies, and enforce performance-oriented coding standards for better overall HPC application performance.} demands further investigation \cite{yeticstiren2023evaluating, godoy2023evaluation, martinez2023code, guo2023longcoder, mukherjee2023stack}. 

%High-Performance Computing (HPC) has emerged as a cornerstone of modern scientific and computational endeavors, enabling tackle increasingly complex and data-intensive problems \cite{reed2022reinventing}.

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%\keywords{Language Models, Code Completion, High-Performance Computing, Fortran, Tokompiler, Polycoder, SPT-Code}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

==> plots/polycoder_completion.tex <==
\begin{figure*}[!ht]
    \centering

    \begin{subfigure}[b]{0.2\textwidth}
\begin{lstlisting}[breaklines=true, breakatwhitespace=true, basicstyle=\footnotesize\ttfamily, columns=fullflexible]
// INPUT (Line 2):
int main (int argc, char *argv[]) {
// COMPLETION:
int i;
int n = argc - 1;
int m = argc - 2;
int k = argc - 3;
int l = argc - 4;
int r = argc - 5;
int c = argc - 6;
int d = argc - 7;
int e = argc - 8;
int f = argc - 9;
int g = argc - 10;
int h = argc - 11;
int i1 = argc - 12;
int i2 = argc - 13;
int i3 = argc - 14;
\end{lstlisting}        
\caption{Given function signature}
        \label{fig:subfig1}
    \end{subfigure}
    %\hspace{0.2cm}
    \hfill
    %
    \begin{subfigure}[b]{0.38\textwidth}
    \begin{lstlisting}[breaklines=true, breakatwhitespace=true, basicstyle=\footnotesize\ttfamily, columns=fullflexible]
// INPUT (Lines 2-10):
int main (int argc, char *argv[]) {
int i,j;  
double x;  
double pi, sum = 0.0; 
double start, delta;  
step = 1.0/(double) steps;
for (j=1; j<= MAX_THREADS; j++) {
printf("running on %d threads: ", j);
omp_set_num_threads(j);  
// COMPLETION:
start = omp_get_wtime();
for (i=0; i<steps; i++) {    
x = (double) i;
pi = 3.141592653589793238
4626433832795028841971693
9937510582097494459230781
6406286208998628034825342
...
    \end{lstlisting}
        \caption{Given initialization}
        \label{fig:subfig2}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[b]{0.38\textwidth}
    \begin{lstlisting}[breaklines=true, breakatwhitespace=true, basicstyle=\footnotesize\ttfamily, columns=fullflexible]
// INPUT (Lines 2-13):
int main (int argc, char *argv[]) {
int i,j;
double x;
double pi, sum = 0.0;
double start, delta;
step = 1.0/(double) steps;
for (j=1; j<= MAX_THREADS; j++) { 
printf("running on %d threads: ", j);
omp_set_num_threads(j);  
sum = 0.0;
double start = omp_get_wtime();  
#pragma omp parallel for reduction(+:sum) private(x) 
// COMPLETION:
for (i=0; i<steps; i++) {
    x = (double) i;
    sum += x;
} ...
    \end{lstlisting}
        \caption{Given context of parallel execution}
        \label{fig:subfig3}
    \end{subfigure}
    \caption{Testing generation of HPC code by the foundation models (PolyCoder example): Evaluating machine-generated text given different contexts of the initial HPC codes and measures the similarity to the true reference.}
    \label{fig:bleutests}
\end{figure*}


